Unsupervised Large Language Model Alignment for Information Retrieval via Contrastive Feedback

Large language models (LLMs) have demonstrated remarkable capabilities across various research domains, including the field of Information Retrieval (IR). However, the responses generated by off-the-shelf LLMs tend to be generic, i.e., cannot capture the distinctiveness of each document with similar content. This limits the performance of LLMs in IR because finding and distinguishing relevant documents from substantial similar documents is a typical problem in many IR tasks. To address this issue, we propose an unsupervised alignment method, namely Reinforcement Learning from Contrastive Feedback (RLCF), empowering LLMs to generate both high-quality and context-specific responses. Our approach constructs unsupervised contrastive feedback signals based on similar document groups, and adopts a reward function, named group-wise reciprocal rank, to optimize LLMs within a standard Proximal Policy Optimization. We conduct extensive experiments to evaluate the effectiveness of RLCF on LLMs built with different languages and parameter sizes on multiple downstream IR applications. RLCF significantly outperforms existing alignment methods, and RLCF-optimized LLMs demonstrate considerable improvement in generating responses with distinctiveness.

==> sections/1_Introduction_new.tex <==
\section{Introduction}
Large Language Models (LLMs) have demonstrated promising performances across a wide range of research fields, such as document summarization~\cite{Reid_2023, liu2023evaluating, huang2023citation, kou2023automated}, information completion~\cite{wu2023survey, gospodinov2023doc2query, wang2023query2doc} and data augmentation~\cite{dai2022promptagator, bonifacio2022inpars}.
% in search engines, LLMs are utilized to generate snippets, or summaries, for retrieved documents~\cite{Reid_2023, liu2023evaluating, huang2023citation, kou2023automated}, aiding users in deciding whether to click on a specific document.
% Additionally, some studies~\cite{wang2021gpl, bonifacio2022inpars,dai2022promptagator} leverage LLMs as tools for data augmentation, generating pseudo-training data to facilitate the performance of dense retrieval models.
% Others~\cite{gospodinov2023doc2query, ma2023pre, wang2023query2doc} utilize LLMs as query or document expansion models to bridge the gap in one another.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pics/summaries_case.pdf}
    \caption{Illustrations of LLMs application in document summarization for similar documents.}
    \label{fig:llminir}
    \vspace{-5mm}
\end{figure}

However, off-the-shelf LLMs tend to generate generic responses for each input with similar content, indicating a deficiency in \textbf{informativeness}. 
Informativeness denotes the degree to which the information provided in the response is comprehensive~\cite{peng2023check,huang2023finbert}.
For instance, Figure~\ref{fig:llminir} show the results of FLAN-T5~\cite{chung2022scaling} when used for document summarization. 
As we can see, the off-the-shelf FLAN-T5 generates the same summary for three different documents with similar content, making them indistinguishable.
Using such summaries as document representations is not acceptable in numerous scenarios, particularly in search engines, due to their inability to aid users in quickly and accurately locating their desired documents.
In information completion, a reasonable yet uninformative completion fails to provide performance gain.
Intuitively, identical items' profile, generated by LLMs for similar items, fails to assist users in selecting their preferred item~\cite{wu2023survey}. 
This challenge corresponds to difficulties encountered in document or query expansion scenarios~\cite{wang2023query2doc, gospodinov2023doc2query}.
Besides, in the data augmentation, a informative pseudo-training sample is also preferred~\cite{dai2022promptagator, bonifacio2022inpars}.
Given the limited ability of LLMs to provide informative responses, their performance in numerous application scenarios is suboptimal.
Therefore, improving the informativeness of LLMs' output emerges a critical challenge.

Recently, alignment techniques~\cite{ouyang2022training,lee2023rlaif,yang2023rlcd,dai2023safe} have attracted significant attention for their remarkable efficacy in improving LLMs with preferred response attributes.
The idea of LLM alignment is to construct feedback to LLM's responses based on the preferred attributes (e.g., helpfulness~\cite{ouyang2022training}, harmlessness~\cite{lee2023rlaif, yang2023rlcd, dai2023safe}, etc.) and use them to optimize LLMs. 
Depending on how the feedback is collected, existing LLM alignments can be broadly categorized into human-based methods and model-based methods. 
Unfortunately, none of the existing alignment methods can be used to improve informativeness of response from LLMs, due to the following limitations:
\begin{itemize}[left=0.1in]
    \item All of existing alignment methods compute feedback in a point-wise manner, i.e., feedback can only be provided to the responses of a single input.
    The distinctions between similar inputs cannot be effectively captured.
    \item While human-based methods such as RLHF~\cite{ouyang2022training} are effective in improving helpfulness and harmlessness, collecting adequate human feedback is expensive and challenging, even for the point-wise manner.
    \item Model-based methods such as RLAIF~\cite{lee2023rlaif} and RLCD~\cite{yang2023rlcd} assume that the feedback model (usually a LLM) is strong enough to construct feedback following a instruction. However, LLMs often fail to provide accurate feedback for informativeness.
\end{itemize}

% \begin{figure}
%     \centering
%     \subfigure[RLHF/RLAIF]{
%         \includegraphics[width=0.45\textwidth]{pics/comparison_RLHF.pdf}
%         \label{fig:rlhf}
%     }
%     \subfigure[RLCD]{
%         \includegraphics[width=0.45\textwidth]{pics/comparison_RLCD.pdf}
%         \label{fig:rlcd}
%     }
%     \subfigure[RLCF]{
%         \includegraphics[width=0.45\textwidth]{pics/comparison_RLCF.pdf}
%         \label{fig:comparison_rlcf}
%     }
%     \caption{Comparison between existing alignment methods and RLCF.}
%     \label{fig:comparison}
%     \vspace{-5mm}
% \end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=6cm]{pics/comparison.pdf}
    \caption{The comparison between existing methods and RLCF. The dotted line represents that the reward score is returned to LLM for PPO optimization.}
    \label{fig:comparison}
    \vspace{-8mm}
\end{figure}

To address these limitations, we propose a novel framework called Reinforcement Learning from Contrastive Feedback (\textbf{RLCF}) to enhance informativeness of LLMs, as shown in Figure~\ref{fig:comparison}. 
RLCF is a \textbf{group-wise} alignment method that constructs feedback for responses generated for a group of similar inputs, and it is fully \textbf{unsupervised}.
Specifically, we first retrieve a group of similar documents for each document in the corpus through a retrieval model. 
Then, the group of similar documents is fed to an LLM to obtain a response for each document. 
The responses could be summaries or any other desired outputs.
Utilizing a reward function named GRR, we construct contrastive feedback from the responses to similar documents.
Finally, the LLM is optimized based on the contrastive feedback using the standard Proximal Policy Optimization (PPO) algorithm~\cite{schulman2017proximal}.

To demonstrate the effectiveness of RLCF, we test it in three representative application scenarios of LLMs that necessitate informativeness: document summarization, document expansion and data augmentation for retrieval.
% The generated query must exhibit specificity to effectively mitigate the false negative issue~\cite{dai2022promptagator, bonifacio2022inpars}, preventing a decline in the effectiveness of data augmentation for dense retrieval models.
% This issue arises due to the presence of a substantial number of similar documents within a corpus, a characteristic frequently observed in IR.
% Insufficient specificity in the generated query may lead to it being interpreted as positive for multiple documents.	
% However, the contrastive loss function permits only a single positive query-document pair during the dense retrieval model training process.
% Consequently, a lack of specificity within the generated query would decrease the effectiveness of data augmentation for dense retrieval models.
% The application of LLMs in the summarization in IR focuses on generating summary for each retrieved document.
% The utilization of LLMs in data augmentation for IR concentrates on the generating queries to train retrieval models.
% Specificity is crucial in all of these scenarios as elaborated in Section~\ref{sec:preliminary}(to be updated in preliminary).
% This specificity helps mitigate the problem of false negatives~\cite{qu2021rocketqa,dai2022promptagator} and enables the precise locating of the preferred document respectively.
% The summaries generated by vanilla LLMs tent to be identical across the retrieved documents, particularly when dealing with similar documents.
% As the retrieved documents are inherently highly similar, a preferred in IR needs to capture distinctions in documents to generate specific summaries, thereby aiding users in conveniently locating the their target document that fulfill their information needs.
% RLCF empowers LLMs to generate distinguishable responses for highly similar documents, thereby enhancing the effectiveness of data augmentation and document summarization in IR.
% With the exponential growth of web documents, the efficient and accurate \textbf{retrieval} and \textbf{selection} of valuable information have acquired increasing attentions, which involve retrieval models and summarization models.
For the evaluation of document summarization, we introduce a automatic metric called Rouge-diff and conduct human evaluation.
To assess the effectiveness of RLCF-optimized LLMs in document expansion and data augmentation, we evaluate the LLMs responses through downstream document retrieval tasks, i.e., comparing the performance retrieval models enhanced by LLM with different alignment methods. 
We perform experiments on both English and Chinese LLMs, with parameters ranging from 770 million to 11 billion.
The LLMs' architectural configurations include encoder-decoder and decoder-only.
The results indicate that, compared to existing alignment methods, RLCF can significantly improve the performance of LLMs in multiple downstream applications necessitating informativeness.
Furthermore, RLCF-optimized LLMs, despite having fewer parameters, could significantly outperform GPT-3.5 and GPT-4.0, which possess much more parameters.

We summarize our main contributions as follows:
\begin{itemize}
    \item We conducted a comprehensive analysis of why LLMs are required to generate informative responses in numerous scenarios, which is elaborated in Section~\ref{sec:dowstream}.
    \item We propose a novel unsupervised framework namely RLCF to enhance the informativeness of LLMs, which is detailed in Section~\ref{sec:method}.
    % \item We are the first to introduce retrieval model into the alignment framework, thereby constructing low-cost, high-quality group-wise contrastive feedback.
    \item As show in Section~\ref{sec:experiments}, the experimental results demonstrate the effectiveness of RLCF on both English and Chinese LLMs as well as various parameter scales and architectures. RLCF outperforms existing alignment methods by a large margin, and RLCF-optimized LLMs could surpass GPT-3.5 and GPT-4.0.
\end{itemize}



==> sections/Method.tex <==
\section{Method}
In this section, we present the details about our proposed framework, Reinforcement Learning from Contrastive Feedback, dubbed as RLCF.
It facilitate LLMs to capture fine-grained distinctions in similar input documents, consequently generating output responses that are more specific.
The overall framework of RLCF is illustrated in Figure~\ref{fig:rlcf}, which comprises two parts.
The blue part in this figure represents data construction for formulating contrastive feedback.
% , as elaborated in Section~\ref{sec:dataConstruction}. 
The green part in this figure outlines the process of optimizing LLMs with the contrastive feedback.
% , with further details provided in Section~\ref{sec:rlcf}. 
In the following, we elaborate the two parts in Sections \ref{sec:dataConstruction} and \ref{sec:rlcf}, respectively.
The commonly used notations are summarized in Table~\ref{table:notation}.
% Afterwards, we present the detailed steps in RLCF, which include unsupervised contrastive data construction and contrastive-based optimization.
% 介绍Figure 3

\begin{table}[]
\caption{The notations used in this paper.}
\label{table:notation}
\begin{tabularx}{0.48\textwidth}{l|X}
\hline\hline
Notations   & Descriptions                                          \\ \hline
$q$           & The query used to search a document.                  \\ \hline
$d$           & A document from corpus.                               \\ \hline
$\mathcal{D}$           & The corpus of documents.                              \\ \hline
$\mathbb{G}_d$          & The similar document group for document d.            \\ \hline
$R_d$          & The response of LLM for document d.                   \\ \hline
$\pi$          & The original parameters of LLM.                       \\ \hline
$\pi_{\phi}^{RL}$   & The optimized RL policy.                              \\ \hline
$\mathcal{R}$           & The reward used to optimize LLM, including the penalty term.                      \\ \hline
Batched-MRR & A variant MRR used for RLCF optimization.                                        \\ \hline
Inst        & An instruction used for few-shot response generation. \\ \hline
Exam        & An example for few-shot response generation.          \\ \hline\hline
\end{tabularx}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pics/rlcf.pdf}
    \caption{The framework of RLCF. The blue part represents the data construction stage of RLCF and the green part represents the RLCF optimization stage. The intersection of these two colors indicates the steps shared between both stages.}
    \label{fig:rlcf}
    \vspace{-5mm}
\end{figure}

% \subsection{Overall Framework}

% The overall framework of RLCF can be formulated as follows:
% \begin{itemize}
%     \item \textbf{Unsupervised Contrastive Data Construction.} We first retrieve the top-K most similar documents from the corpus by an unsupervised dense retrieval model to construct a group of similar documents. Then, we generate a response for each document in the group constructed in the previous step using large language models. The responses could be a query or a summary for their corresponding documents.
%     \item \textbf{Contrastive-based Optimization.} Subsequently, contrastive feedback is obtained through an unsupervised dense retrieval model called Contriever. 
%     Specifically, Contriever takes the documents and their responses generated by LLMs as input to compute the contrastive feedback using the Mean Reciprocal Rank (MRR) within the batch. Finally, the optimization of LLMs is achieved through contrastive feedback using the Proximal Policy Optimization (PPO) algorithm, a widely employed reinforcement learning framework.
% \end{itemize}

% Figure~\ref{fig:rlcf} illustrates the overall framework of RLCF.
% We refer to this framework as RLCF since LLMs are optimized through contrastive feedback using the PPO algorithm, a type of reinforcement learning framework. 
% It is noteworthy to mention that this entire framework operates without supervision, thereby eliminating the need for costly human labeling overhead.
% Next, we present the comprehensive definition of each step in RLCF and elaborate how the framework aligns the capabilities of LLMs with the requirements of IR.

\subsection{Contrastive Data Construction}
\label{sec:dataConstruction}
To facilitate the capacity of LLMs for capturing subtle distinctions among documents, we first propose to create groups of similar documents
% that are challenging for vanilla LLMs to distinguish.
to obtain contrastive feedback.
These feedback signals contribute to he optimization of LLMs, enabling it to extract fine-grained distinction from similar documents, which is elaborated in Sec.~\ref{sec:rlcf}. 
In particular, the similar document groups are constructed by an unsupervised retriever, such as a \textit{dense retrieval model}, to avoid the high cost of data labeling.
In this subsection, we introduce the details about how to construct contrastive data for RLCF optimization.

\noindent\textbf{Similar Documents Retrieval.}
% As contrastive feedback is derived from comparing similar documents, the initial step of data construction involves constructing groups of similar documents. 
As contrastive feedback relies on the comparison of similar documents, the initial step of data construction involves forming groups of similar documents.
We utilize a retriever to retrieve similar documents for a given document.

Formally, we retrieve the top-K most similar documents to form the similar document group $\mathbb{G}$ for a given document $d$ in the corpus $\mathcal{D}$. 
% Each document is limited to the first 512 tokens, and any tokens beyond 512 are truncated.
% More specifically, we encode each document $d\in \mathcal{D}$ through Equation~\ref{eq:encodeT}.
The similar document group $\mathbb{G}_{d_i}$ for document $d_i$ is defined as
\begin{equation}
    \label{eq:group}
    \mathbb{G}_{d_i} = \{d_j~|~\underset{\text{top-}\mathrm{K}}{\mathrm{argmax}}\ S\left(d_i, d_j\right), \forall d_j \in \mathcal{D}, i\neq j\}.
\end{equation}
Here, $S(d_i, d_j)$ denotes the similarity score between $d_i$ and $d_j$. 
Table a standard duel-encoder based dense retrieval model as an example, the similarity between documents are computed as
\begin{equation}
    \label{eq:similarity}
    S(d_i, d_j)=E_{d_i}\cdot E_{d_j},
\end{equation}
where the $\cdot$ means the inner production operation. 
$E_{d}$ denotes the embedding of document $d$, which is the average pooling of the last layer's token representation after the encoding of retriever $\mathrm{M}$, as defined in the following,
\begin{equation}
    \label{eq:encodeT}
    E_d = \mathrm{Avg\_Pooling}\left(\mathrm{M}\left(d\right)\right).
\end{equation}


\noindent\textbf{Response Generation.}
With a similar documents group, we use LLMs to generate responses for each document within the group $\mathbb{G} = \left\{d\cup\mathbb{G}_d\right\}$. 
These responses could be queries or summaries, serving purposes such as data augmentation or summarization.

Formally, we take the concatenation of instruction denoted as $\mathrm{Inst}$, several examples denoted as $\mathrm{Exam}$ and the document $d\in\mathbb{G_d}$ as input to perform few-shot response generation. The examples $\mathrm{Exam}$ are randomly chosen from human-labeled data specific to a particular task.
This process can be defined as
\begin{equation}
    \label{eq:llm}
    R_d = \mathrm{LLM}\left(\mathrm{Inst}\oplus \mathrm{Exam} \oplus d\right).
\end{equation}
Here, $\oplus$ represents the concatenation operation.
Since the search intent of each task for IR is different, we refer to the previous study~\cite{dai2022promptagator} and design a specific instruction for each task.
The prompt templates are presented in Appendix~\ref{sec:prompt}.

% For document summarization, we only use instruction $\mathrm{Inst}$ and document $d\in\mathbb{G_d}$ as the input of LLMs to conduct zero-shot document summarization. Therefore, Equation~\ref{eq:llm} could be rewritten as
% \begin{equation}
    % \label{eq:llm_sum}
    % R_d = \mathrm{LLM}\left(\mathrm{Inst}\oplus d\right).
% \end{equation}

Finally, the document $d\in \mathbb{G}$ and the generated response $R_d$ are utilized in Equation (\ref{eq:batched-mrr}) for contrastive feedback calculation, which is then utilized in the subsequent RLCF optimization process.




\subsection{RLCF Optimization}
\label{sec:rlcf}
Next, we introduce the calculation of contrastive feedback, which serves as the reward score in RLCF.
The reward score represents the degree to which the environment prefers the responses generated by LLMs.	
% RLHF~\cite{ouyang2022training} demonstrates that it is effective in aligning the outputs of LLMs with human preferences, providing valuable insights into alignment techniques of LLMs.
% However, RLHF requires a substantial amount of supervised preference data  for training a reward model, which is challenging and expensive to get.
To circumvent the high cost of human labeling, RLCF proposes to leverage an unsupervised retrieval model to replace the reward model used in RLHF~\cite{ouyang2022training}, as depicted in Figure~\ref{fig:rlcf}.
The contrastive feedback is a variant of Mean Reciprocal Rank (MRR), a widely used metric in IR, which is defined as
\begin{equation}
    \label{eq:mrr}
    MRR@K = \frac{1}{|\mathcal{Q}|}\sum_{q\in \mathcal{Q}}\frac{\mathbf{I}(rank\leq K)}{rank}.
\end{equation}
Here, $\mathbf{I(\cdot)}$ is a indicator function. The $rank$ in Equation (\ref{eq:mrr}) denotes the position of the \textit{first} relevant document in the retrieved candidates of query $q$ and $\mathcal{Q}$ is the query collection of a evaluation set.

Given that the candidates of query $q$ is retrieved from the whole corpus, the traditional MRR is a corpus level metric.
Therefore, the computational overhead could be magnified by the scale of massive corpus and eventually cause unacceptable efficiency degeneration of model optimization.
To address this issue, we introduce Batched-MRR, a variant MRR computed in the batch level.
Considering that the most similar documents are already grouped in data construction process (as elaborated in Section~\ref{sec:dataConstruction}) and are subsequently fed into the same batch, Batched-MRR can be viewed as an approximation of MRR, since the documents that most affect the output of indicator function $\mathbf{I(\cdot)}$ in Equation (\ref{eq:mrr}) are almost within a batch.
The calculation of Batched-MRR can be defined as
\begin{equation}
    \label{eq:batched-mrr}
    \textrm{Batched-MRR}_{R_d} = \frac{1}{rank}.
\end{equation}
Here, $rank$ represents the position of a document $d$ within a batch, which is sorted by a retriever based on the similarity score $S(d, R_d)$ against the response $R_d$ generated by an LLM. 
% The similarity score, denoted as $S(d, R_d)$, is computed using Equation~\ref{eq:similarity}.
% To calculate the similarity score $S(\cdot)$, the retriever $\mathrm{M}$ first encodes the text $t$ into a representation, which can be defined as 
% \begin{equation}
%     \label{eq:encodeT}
%     E_t = \mathrm{Avg\_Pooling}\left(\mathrm{M}\left(t\right)\right),
% \end{equation}
% where $E_{t}$ denotes the average pooling of the last layer's token representation. The text $t$ could be a document $d$ or a response $R_d$. 
% Then, the similarity score $S(\cdot)$ is calculated as
% \begin{equation}
%     \label{eq:similarity}
%     S\left(\mathbf{d}, \mathbf{R_d}\right)=E_{d}\cdot E_{R_d},
% \end{equation}
% where the $\cdot$ means the inner production operation.


\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{pics/ppo.pdf}
    \caption{The comparison between RLHF and RLCF. The dotted line represents that the reward score is returned to LLMs for PPO optimization.}
    \label{fig:ppo}
    \vspace{-5mm}
\end{figure}
Our objective is to optimize the policy model, i.e., the LLM, using contrastive feedback to generate responses that are desired in the context of IR.
We achieve this through reinforcement learning, specifically with the PPO~\cite{schulman2017proximal} algorithm.
We consider the Batched-MRR as the reward score for the entire response, and maximize it using the PPO algorithm.
Following with prior study~\cite{ouyang2022training}, we also incorporate a term in the reward that penalizes the KL divergence between the optimized RL policy $\pi_{\phi}^{RL}$ with parameters $\phi$ and the original large language model $\pi$. 
The penalty term prevents the policy model from producing responses that diverge significantly from the vanilla LLM, thereby preserving the language capabilities of the policy model.
The full reward $\mathcal{R}$ could be written as
\begin{equation}
\label{eq:ppo_reward}
\mathcal{R}(d, R_d)=\textrm{Batched-MRR}_{R_d}-\beta \log \left[\pi_\phi^{\mathrm{RL}}(R_d \mid d) / \pi(R_d \mid d)\right],
\end{equation}
where $\beta$ is a hyper parameter that balances the Batched-MRR and penalty term.

\noindent\textbf{Remarks.} 
RLHF~\cite{ouyang2022training} demonstrates that it is effective in aligning the outputs of LLMs with human preferences, providing valuable insights into alignment techniques of LLMs.
However, RLHF requires a substantial amount of supervised preference data  for training a reward model, which is challenging and expensive to get.
Figure~\ref{fig:ppo} shows the difference between RLHF and our proposed RLCF framework. First, instead of directly using a reward model, RLCF employs an unsupervised retrieval model to obtain a reward score by comparing documents within a batch, where the in-batch documents are highly similar.
% . Notably, the documents within the same batch are highly similar.
% The details of contrastive data construction are presented in Section~\ref{sec:dataConstruction}.
% Figure~\ref{fig:ppo} 
Second, the rewards in RLCF are obtained at the batch level, whereas in other frameworks like RLHF, rewards are obtained at the single document level, which cannot help LLMs to distinguish different documents. Most importantly, the reward model in RLHF demands a substantial amount of human-labeled samples for training to obtain an effective reward score for aligning LLMs with a desired attribute. In contrast, our RLCF framework does not require any additional human labeling, which is more practical to be used.



